Neural Network Robustness as a Verification Property: A Principled Case Study

Neural networks are very successful at detecting patterns in noisy data, and have become the technology of choice in many fields. However, their usefulness is hampered by their susceptibility to adversarial attacks. Recently, many methods for measuring and improving a network's robustness to adversarial perturbations have been proposed, and this growing body of research has given rise to numerous explicit or implicit notions of robustness. Connections between these notions are often subtle, and a systematic comparison between them is missing in the literature. In this paper we begin addressing this gap, by setting up general principles for the empirical analysis and evaluation of a network's robustness as a mathematical property - during the network's training phase, its verification, and after its deployment. We then apply these principles and conduct a case study that showcases the practical benefits of our general approach.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

%From their inception in the first half of the 20th century, to their rise in computer vision and signal processing applications in the 90s, neural networks have made their way into modern AI applications, mostly as components responsible for perception tasks, e.g. processing signals, images, speech or text.

%Unfortunately, neural networks lack properties known as \emph{explainability} and \emph{interpretability}:  we usually deploy them in domains where the ideal data distribution is unknown or unattainable. Therefore, by definition, they are only approximately correct, only as good as the data is, and do not carry  additional semantic meaning beyond a very general type $\real^n \rightarrow \real^m$. In the absence of a clear specification, it becomes problematic to guarantee the absence of ``bugs'', or identify components that are responsible for deviations from the intended behaviour.


Safety and security are critical for some complex AI systems involving neural networks, yet they are difficult to ensure.
%, the question of their safety and security comes to the forefront.
The most famous instance of this problem is guaranteeing robustness against \emph{adversarial attacks}~\cite{intriguing_properties_of_neural_networks_2014_szegedy,GoodfellowSS14}.
%The \emph{$\epsilon$-ball robustness}
%is widely used in the literature~\cite{SinghGPV19,HuangKWW17,KatzHIJLLSTWZDK19}.
Intuitively, an image is \emph{$\epsilon$-ball robust} if, when you move no more than~$\epsilon$ away from it in the input space,  the output does not change much, or alternatively, the classification decision that the network gives does not change. %.moves no more than $\delta$ in the output space.
%
%To ensure that the network is robust for a given dataset, we must ensure that the network is robust in the vicinity of each of the given images.
%Let us now look at the existing solutions to this problem from the formal point of view.
\emph{Adversarial robustness} is a property that even very accurate neural networks fail to satisfy.

%their verification has become a hot topic, with several competing tools and methods on the market: ERAN~\cite{GeMiDrTsChVe18}, Marabou~\cite{KatzHIJLLSTWZDK19}, nnenum~\cite{bak2020improved} to name a few.
%However, verification tools do not entirely solve the problem as they do not directly address the issue of an under-defined specification during training. To put it plainly, there is no reason to run a computationally expensive verifier if the neural network is not robust in the first place.

The proposed solution is to (re)train the network with robustness specifically in mind. 
Such training can be seen as a way to impose a formal specification, and so may contribute to explainability as well as verification.
This work considers four of the most prominent families of training techniques:
\begin{enumerate}
\item \emph{Data augmentation}~\cite{ShortenK19}
\item \emph{Adversarial training}~\cite{GoodfellowSS14,madry2018towards}
\item \emph{Lipschitz robustness training}~\cite{anil2019sorting,pauli2021training}
\item \emph{Training with logical constraints}~\cite{XuZFLB18,FischerBDGZV19}
\end{enumerate}
The last technique, \emph{training with logical constraints}, is a more general approach that can train for not just robustness, but a wide range of constraints expressed in some logical language.

Although the first three families of methods all seek to represent the same high-level knowledge in the neural network, each technique seeks to optimise for subtly different definitions of robustness. We formally identify these as
\emph{standard} (SR), \emph{classification} (CR),  \emph{Lipschitz} (LR) and \emph{strong classification} (SCR) robustness. Given these differences, some natural questions to ask are: What are the relationships between them? What assumptions do they make about the training dataset? Are some more effective than others? Are some more interpretable by users than others?

\textbf{Contributions.}
In this work, we attempt to answer these questions. We take classification problems as an example domain, interpreting a neural network ${f : \real^n \rightarrow \real^m}$ as a procedure that separates the $n$-dimensional data into $m$ classes.  This enables the following findings: 
%
%\begin{itemize}
%
%\item
  We observe that from the security perspective, different definitions of robustness ultimately determine the nature of attack,
  thus giving rise to SR, CR, LR, SCR attacks. Thus, one can train for example with SCR constraint but attack with SR constraint.
  This raises questions about relative strengths of these different training methods and attacks.
%
%\item
  Some constraint-driven training methods are special cases of others.
  For example, adversarial training known in the literature can be seen as a form of training with SR constraint, with certain amount of parameter tuning.

 % 
%\item
  We can order some robustness constraints based on their strength, for example, we show that LR \emph{implies} SR, and SCR \emph{implies} CR.
  In this case, training with a stronger constraint (e.g. LR) will protect better against both kinds of attacks (in this case, both SR and LR attacks).
%
%\item
  Some pairs of constraints cannot be ordered by strength (e.g. SR and SCR, LR and SCR), and in this case, optimising training for a given constraint defends better only against attacks with this same target constraint.
%
%\item
  Moreover, we show that training with logical constraints defends against adversarial attacks better than data augmentation for any choice of robustness definition as a training constraint.  
%
%\item
 Finally, we show that there are additional common criteria that can be used to qualitatively compare different modes of constraint-driven training, e.g. interpretability, global or local nature. E.g. CR is the most interpretable, but not globally desirable, LR is least interpretable, but globally desirable.   
 % \end{itemize}

%perform an in-depth study of the differences between these definitions, comparing their relative power,
%define common metrics for relative evaluation of these different notions of robustness:
%interpretability, expressivity, verifiability, and in-built assumptions. We highlight that these differences have real consequences: for example, data augmentation makes strong assumptions about where on the data manifold the training dataset is distributed. 



\begin{comment}
In Section~\ref{sec:experiments},
%we first answer the above question empirically, by subjecting three kinds of networks above to an FGSM attack.
we conduct a series of experiments that compare relative performance of these methods based on their resistance to a PGD-based adversarial attacker, and find that:
\begin{itemize}
\item[\textbf{E1.}]  Generally, optimising training for a given constraint defends better against attacks that target that constraint.  
And yet, for any kind of attack, there is a choice of a training constraint that defends better against this attack;
\item[\textbf{E2.}] Training with logical constraints defends against adversarial attacks better than data augmentation for any choice of robustness definition as a training constraint;
\item[\textbf{E3.}]
In terms of defence against unknown attacks, neural networks that use the Lipschitz robustness constraint for training performs better than those trained with any other available constraint;
\item[\textbf{E4.}] some forms of robustness are harder to achieve: e.g. ``standard robustness'' is consistently higher than ``approximate classification robustness'', for any training regime.   
\matthew{What does ``consistently higher" mean?}
% and is almost on par with adversarial training.
\end{itemize}
\end{comment}

To our knowledge, this is the first systematic study of robustness training from
the point of view of the impact of precise formalisation of robustness on training, evaluation and attack.
Note that some of the previous work reported on unstable performance of constraint-driven training when defending against attacks~\cite{AEHW20}, which we do not observe in our experiments. 
 %\matthew{Again, we ``disprove" is strong. ``We do not observe" perhaps?}
Some papers~\cite{FischerBDGZV19} listed and even implemented some kinds of robustness constraints that we study here,
but gave no indication of their relative performance. We are not aware of any prior analysis of SR, LR, CR, SCR abstractly as logical constraints.
%We are confident that this general method of initial abstract constraint analysis followed by subsequent application to
%training and evaluation of networks will be of use beyond classification algorithms and robustness constraints.   
%, and no discussion of the expected or relative properties of the trained networks from the knowledge representation point of view. 


%a general ``knowledge representation'' point of view.
%Although robustness was chosen as the constraint of interest in this paper, we aim to convincingly illustrate that training using logical constraints generally requires careful formal treatment, as many misconceptions and even errors arise on the boundary between logical constraints (such as the definitions of robustness expressed in~\cite{FischerBDGZV19}) and their machine-learning realisations (given by explicit or implicit translation into the language of loss functions and statistical optimisation). At the same time, this paper aims to convince the reader that conceptual clarity in this domain is possible; and thus aims to open new possibilities for a future community project on formally expressing and analysing other properties of machine-learning algorithms.

The paper is organised as follows. Section~\ref{sec:robustness-training} explains how different robustness constraints arise from different machine learning approaches to constraint-driven training. Section~\ref{sec:robustness-definitions}  abstractly analysises these robustness definitions, establishing their relative strength, interpretability and applicability. Section~\ref{sec:experiments} shows how these robustness constraints determine different evaluation metrics and attacks, and provides a comprehensive empirical evaluation of the robustness constraints deployed as training constraints and as attacks. Section~\ref{sec:concl} concludes the paper and outlines future work.




%\katya{NB, in an attempt to introduce complex notions using intuitive terms, I am saying that a definition of robustness determines our understanding of an attack. Do you agree? Example: of I use definition of SCR, then for me an attack is when the NN's class prediction changes.}

%limitations of the popular method of ``constraint-driven training'' from the verification point of view. Its  aim is two-fold: to warn the community of existing and potential pitfalls, but to also provide more clues to the design of future methods of continuous verification. In particular, one take away lesson is that such systems should be more transparent in showing various settings that work behind the scenes to translate logical constraints. It seems likely that the ability to tune and adjust these settings will be crucial in advancing continuous verification.


==> sections/marabou.tex <==
\section{Marabou}
\label{sec:marabou}

\begin{table}[t]
\centering
\caption{\emph{\footnotesize{Constraint satisfaction results for the Classification, Standard and Lipschitz Constraints queries.}}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|llll|llll|}
\hline
 & \multicolumn{4}{l|}{FASHION} & \multicolumn{4}{l|}{GTSRB} \\ \hline
 Networks &
  \multicolumn{1}{l|}{Baseline} &
  \multicolumn{1}{l|}{SCR} &
  \multicolumn{1}{l|}{SR} &
  LR &
  \multicolumn{1}{l|}{Baseline} &
  \multicolumn{1}{l|}{SCR} &
  \multicolumn{1}{l|}{SR} &
  LR \\ \hline
Classification Constraint &
  \multicolumn{1}{l|}{1.5\%} &
  \multicolumn{1}{l|}{2\%} &
  \multicolumn{1}{l|}{2\%} &
  34\% &
  \multicolumn{1}{l|}{0.5\%} &
  \multicolumn{1}{l|}{1\%} &
  \multicolumn{1}{l|}{3\%} &
  4.5\% \\ \hline
Standard Constraint &
  \multicolumn{1}{l|}{0.5\%} &
  \multicolumn{1}{l|}{1\%} &
  \multicolumn{1}{l|}{65.83\%} &
  100\% &
  \multicolumn{1}{l|}{0\%} &
  \multicolumn{1}{l|}{0\%} &
  \multicolumn{1}{l|}{24\%} &
  97\% \\ \hline
Lipschitz Constraint &
  \multicolumn{1}{l|}{0\%} &
  \multicolumn{1}{l|}{0\%} &
  \multicolumn{1}{l|}{0\%} &
  0\% &
  \multicolumn{1}{l|}{0\%} &
  \multicolumn{1}{l|}{0\%} &
  \multicolumn{1}{l|}{0\%} &
  0\% \\ \hline
\end{tabular}%
}
\label{tab:marabou_results}
\end{table}

In this Section we present the constraint satisfaction results (Table~\ref{tab:marabou_results}) that we obtained using the verification framework Marabou~\cite{marabou}.

The networks used in this experiments consist of two fully connected layers: the first one having 30 neurons and ReLU as activation function, and the last one having 10 neurons.

We evaluate them on two benchmark datasets:
\begin{enumerate}
\item The \emph{FASHION MNIST} (or just \emph{FASHION}) dataset~\cite{fashionmnist}  consists of $28 \times 28$ greyscale images of clothing items; 60,000 for training and 10,000 for testing. It has 10 classes: T-shirt/top, Trouser, Pullover, Dress, Coat, Sandal, Shirt, Sneaker, Bag, Ankle boot.
\item The \emph{GTSRB} dataset~\cite{gtsrb} contains $50,000$ images of German traffic signs. There are 40 classes and image sizes vary between $15 \times 15$ to $250 \times 250$ pixels. We use a modified version here that contains $12,660$ training images and $4,170$ test images. These images are all centre-cropped, greyscaled, $48\times 48$ pixel and belong to 10 classes.
\end{enumerate}

Additionally, for each dataset, we train four networks:
\begin{enumerate}
\item The \emph{baseline} network, trained just with cross-entropy.
\item The \emph{SCR} network, trained using the \emph{SCR} constraint with $\alpha = 1$, $\beta = 0.2$, $\epsilon = 0.1$, $\eta = 0.52$ and $L^{\infty}$.
\item The \emph{SR} network, trained using the \emph{SR} constraint with $\alpha = 1$, $\beta = 0.2$, $\epsilon = 0.1$, $\delta = 10$ and $L^{\infty}$.
\item The \emph{LR} network, trained using the \emph{LR} constraint with $\alpha = 1$, $\beta = 0.2$, $\epsilon = 0.1$, $L = 10$ and $L^{\infty}$.
\end{enumerate}

Finally, we define three queries to evaluate constraint satisfaction on: Classification, Standard and Lipschitz Constraints as defined in Section~\ref{sec:robustness-training} with $\alpha = 1$, $\beta = 0.2$, $\epsilon = 0.1$, $\delta = 10$, $L = 10$ and $L^{\infty}$ distance metrics.

Table~\ref{tab:marabou_results} confirms our previous results.
The Lipschitz constraint is the hardest to satisfy and indeed we have 0 images verified.
The networks trained with the LR constraint hugely improve on Standard and Classification constraints queries over the others.
SCR networks do not show any significant improvement over the Baselines on constraint satisfaction.




















